Radio detection in the multi-messenger context

The present work discusses the development of the radio technique for detection of ultra-high energy air-showers induced by cosmic radiation, and the prospects of its application in the future multi-messenger activities, particularly for detection of ultra-high energy cosmic rays, gamma rays and neutrinos. It gives an overview of the results achieved by the modern digital radio arrays, as well as discuss present challenges and future prospects.}

==> Makefile <==
FILE = kostunin-vlvnt2018 

PDFLATEX = pdflatex
BIBTEX = bibtex

PDF = ${FILE}.pdf

.tex.pdf :
	${PDFLATEX} ${FILE}.tex
	${BIBTEX} ${FILE}
	${PDFLATEX} ${FILE}.tex
	${PDFLATEX} ${FILE}.tex

bib :
	${PDFLATEX} ${FILE}.tex
	${BIBTEX} ${FILE}
	
pdf : bib
	${PDFLATEX} ${FILE}.tex
	${PDFLATEX} ${FILE}.tex

# Various cleaning options
clean :
	/bin/rm -f  *.log *.aux *.dvi *.bbl *.blg *.bm *.toc *.out \
	*Notes.bib *.ps

